An App Performance Optimization Advisor for Mobile Device App Marketplaces

On mobile phones, users and developers use apps official marketplaces serving as repositories of apps. The Google Play Store and Apple Store are the official marketplaces of Android and Apple products which offer more than a million apps. Although both repositories offer description of apps, information concerning performance is not available. Due to the constrained hardware of mobile devices, users and developers have to meticulously manage the resources available and they should be given access to performance information about apps. Even if this information was available, the selection of apps would still depend on user preferences and it would require a huge cognitive effort to make optimal decisions. Considering this fact we propose APOA, a recommendation system which can be implemented in any marketplace for helping users and developers to compare apps in terms of performance. APOA uses as input metric values of apps and a set of metrics to optimize. It solves an optimization problem and it generates optimal sets of apps for different user's context. We show how APOA works over an Android case study. Out of 140 apps, we define typical usage scenarios and we collect measurements of power, CPU, memory, and network usages to demonstrate the benefit of using APOA.

==> Makefile <==
NAME=main
BIBTEX=bibtex
LATEX=latex
PDFLATEX=pdflatex
VIEWER=`cat ~/.viewer || which okular || which evince || which open`
LATEX_OPTS=-interaction=nonstopmode -halt-on-error
TEXS=$(shell ls *.tex)
VPATH=.:figures:figs:autofigs

FIGS=$(shell ls images/*.eps) \
	$(shell ls images/*.jpg) 




JPGS=$(patsubst %.jpg,%.eps,$(filter %.jpg,$(FIGS)))
GIFS=$(patsubst %.gif,%.eps,$(filter %.gif,$(FIGS)))
PNGS=$(patsubst %.png,%.eps,$(filter %.png,$(FIGS)))
SVGS=$(patsubst %.svg,%.eps,$(filter %.svg,$(FIGS)))
PDFS=$(patsubst %.pdf,%.eps,$(filter %.pdf,$(FIGS)))

EPSS=$(addsuffix .eps,$(basename $(FIGS)))


.PHONY: all clean default view push commit zip

default: view

all: $(NAME).pdf

# # From PS
# $(NAME).pdf: *.cls $(NAME).tex *.bib $(EPSS)
# 	echo $(EPSS)
# 	$(LATEX) $(LATEX_OPTS) $(NAME).tex
# 	@if(grep "There were undefined references" $(NAME).log > /dev/null);\
# 	then \
# 		$(BIBTEX) $(NAME); \
# 		$(LATEX) $(LATEX_OPTS) $(NAME).tex; \
# 	fi
# 	@if(grep "Rerun" $(NAME).log > /dev/null);\
# 	then \
# 		$(LATEX) $(LATEX_OPTS) $(NAME).tex;\
# 	fi
# 	$(LATEX) $(LATEX_OPTS) $(NAME).tex
# 	dvips -j0 -Ppdf -Pbuiltin35 -G0 -z $(NAME).dvi
# 	gs -q -dPDFA \
# 	-dNOPAUSE -dBATCH -dSAFER -dPDFSETTINGS=/prepress \
# 	-dAutoFilterColorImages=false \
# 	-dAutoFilterGrayImages=false \
# 	-dAutoFilterMonoImages=false \
# 	-dColorImageFilter=/FlateEncode \
# 	-dGrayImageFilter=/FlateEncode \
# 	-dMonoImageFilter=/FlateEncode \
# 	-sDEVICE=pdfwrite -sOutputFile=$(NAME).pdf \
# 	-c .setpdfwrite \
# 	-f $(NAME).ps
# 
# from PDF
$(NAME).pdf: *.cls $(NAME).tex *.bib $(PDFS) $(TEXS)
	echo $(EPSS)
	$(PDFLATEX) $(LATEX_OPTS) $(NAME).tex
	@if(grep "There were undefined references" $(NAME).log > /dev/null);\
	then \
		$(BIBTEX) $(NAME); \
		$(PDFLATEX) $(LATEX_OPTS) $(NAME).tex; \
	fi
	@if(grep "Rerun" $(NAME).log > /dev/null);\
	then \
		$(PDFLATEX) $(LATEX_OPTS) $(NAME).tex;\
	fi
	$(PDFLATEX) $(LATEX_OPTS) $(NAME).tex

clean:
	rm *.blg *.bbl *.log *.aux $(NAME).pdf $(NAME).dvi $(NAME).ps || echo Already Clean

view:	$(NAME).pdf
	$(VIEWER) $(NAME).pdf

$(SVGS) : %.eps : %.svg
	inkscape -b white -t -T --export-ignore-filters --export-eps=$@ $<

# Use PS pipeline for maximum compatibility with random latex packages

$(JPGS) : %.eps : %.jpg
	anytopnm $< | pnmtops -nocenter -equalpixels -dpi 72 -noturn -rle -setpage - > $@
$(GIFS) : %.eps : %.gif
	anytopnm $< | pnmtops -nocenter -equalpixels -dpi 72 -noturn -rle -setpage - > $@
$(PNGS) : %.eps : %.png
	anytopnm $< | pnmtops -nocenter -equalpixels -dpi 72 -noturn -rle -setpage - > $@



%-crop.pdf: %.pdf
	pdfcrop $<

$(PDFS) : %.eps : %.pdf
	pdftops -eps $< $@

push:	commit
	git push

commit:	
	git commit -av

zip : $(NAME).zip

$(NAME).zip : *.cls $(NAME).tex *.bib $(EPSS) Makefile
	zip $@ $^

x: $(NAME).pdf
	xournal $(NAME).pdf


==> preferences.tex <==
In \cite{falaki_diversity_2010} authors analyze detailed usage traces from 255 users of Android and Windows smartphone platforms, with 7-28 weeks of data per user. They report that user diversity is an overarching theme in their findings. Specifically they conclude that different users interact with their phones 10-200 times a day on average and the mean interaction length of different users is 10-250 seconds. The interaction time is between 30 and 500 minutes in a day. %Individual users interact with their smartphone anywhere between 10 to 200 times a day on average. For any given user, most of the sessions are short but some are very long. The median session length is less than a minute but some are longer than an hour.
A similar study is done in \cite{oliver_challenges_2010} where the author collects and studies thousands of traces from over 17,300 BlackBerry users around the world. He obtains a similar trend and reports more precise numbers. Specifically the author finds that the median number of daily interactions is 76 (on average of 86.9 times per day) with a median total interaction time of 1.31 hours (on average 1.68 hours per day). In addition to the previous, authors also study in \cite{falaki_diversity_2010} the apps usage and they report that the median number of apps used by users is roughly 50 although it does not mean that they use them equally. Authors find that users devote the bulk of their attention to a subset of apps of their choice. To provide an aggregate view of what users use their smartphones for they categorize apps into eight different categories and they conclude that communication and browsing dominate and maps, media, and games have a comparatively lower but nevertheless substantial share of user attention. %An overwhelming majority, close to 90\%, of interactions include only one application. That interaction sessions very often have only one application session suggests that users tend to interact with their smartphone for one task at a time, and most of these tasks require the use of only one application. Anyway, different application types have different session lengths.

%We uncover a surprising level of diversity among smartphone users. For almost every aspect of usage that we study, we find one or more orders of magnitude difference between users. Our findings strongly motivate the need for customizing smartphones to their users. We believe that this need is greater than that for customizing ordinary cellphones or laptops. User diversity motivates adapting to the smartphone user.

Both studies observe wide variation among users' daily interaction and this extent of user diversity implies that mechanisms that work for the average case may be ineffective for a large fraction of the users. From these studies we conclude that the context of usage is important and we motivate the need for customizing smartphones to their users and context. In this section we define different contexts of usage and we explain how APOA can be adapted to consider user preferences to solve the Android Selection Problem.

\ruben{Different contexts different objectives and, therefore, different instances of the Android Selection Problem.}

\ruben{If some categories are not important for the user they can be removed and a new Android Selection Problem will be defined considering the important ones.}

\ruben{If some categories are more important than others, weights could be introduced.}

\ruben{Once a Pareto front is generated decision making could applied to choose the most preferred solutions. For example, filtering out solutions which do not satisfy some requirements.}

%In this section, we survey 20 Android users to get information about contexts of use. In addition we monitor their mobile phones for two weeks and we analyze how they use Android apps and how often they change between apps belonging to different categories. We do this installing in their mobile phones App Usage-Manage/Track Usage\footnote{https://play.google.com/store/apps/details?id=com.a0soft.gphone.uninstaller\&hl=en}, an Android app to track apps usage. We choose this app because (1) it is free and it is available in the official Android marketplace, (2) it runs in background and it is not annoying for the user, (3) it generates statistics about use time of installed apps and a time-line of apps usage, and, because, (4) information can be exported to a CSV file to be easily processed. %\mbox{Figure  \ref{fig:appUsage}} shows an example of the list of apps used for one of the authors in a day (November 3, 2016). As it is shown, the phone was used 1h. 44m. 51s. and most of the time (41\%) the browser was used. This kind of information for 20 users and during two weeks will be collected and processed to analyze how often they use Android apps and how often they change between apps belonging to different categories.

%\begin{figure}[H]
%\centering
%\includegraphics[scale=0.2]{images/appUsage.jpg}
%\caption{Screenshot of App Usage-Manage/Track Usage Android app. It shows statistics about total use time of Android apps.}
%\label{fig:appUsage}
%\end{figure}
%
%In addition to the previous, we plan to survey these Android users to get information about different context of usage and the importance of the metrics considered in this work, which are described in \mbox{Section \ref{sec:selectionproblem}}.

%We select 20 different participants considering different occupations (students and workers), ages, and sexes (males and females). We install the track usage Android app in their Android phones and we collect data about usage of apps for two weeks (covering two weekends). The only information we give to the participants is the information collected by this tracker app, but we do not give them any details about the research goal to avoid any bias. After two weeks we survey participants asking about contexts of use and about the importance of performance metrics.

\begin{enumerate}
\item{Travel abroad. This context considers users who travel abroad (for working or holidays). In that case we consider that most important performance metrics are battery life (because likely the time between consecutive charges is longer) and network usage (given that data roaming is usually expensive). Instance eight of the Android Selection Problem.}
\\

\item{Old devices. As we mention in \mbox{Section \ref{sec:introduction}}, a lot of Android users own old devices which are limited in terms of CPU and RAM memory. Therefore, in this context we consider that the most important performance metrics are CPU and memory usages (because if apps are CPU and/or memory greedy the device slows down impacting negatively the user's experience). Instance 10 of the Android Selection Problem.}
\\

\item{Driving. This context include users who use their mobile devices as GPS navigator. At this point we divide this context in two different subcontexts.}

\begin{itemize}
\item{Phone is plugged to the car charger. In this case we consider that the most important performance metric is the network usage (to minimize data plan usage), and CPU and memory usages (to avoid lags in navigation due to the phone's slow down). Instance eight of the Android Selection Problem. Instance 22 of the Android Selection Problem.}
\item{Phone is not plugged to the car charger. Here energy consumption is the most important performance metric to be optimized. Instance one of the Android Selection Problem.}
\end{itemize}
\end{enumerate}

\subsection{Frequency of usage.}

\begin{itemize}
\item{How many apps' categories do usually Android users use?}
\item{How much time apps belonging to each category are used?}
\item{How often do users change between different apps' categories?}
\end{itemize}

\subsection{Considering user preferences in the Android Selection Problem}
Once user preferences are known, this information can be taken into account in the optimization problem. Basically this can be done in three ways, which are described next.

\subsubsection{Handling preferences as constraints in the problem}
Preferences are considered before the optimization problem is solved. It is known as ``a priori'' methods. 

\subsubsection{Preference-based EMO algorithms}
Preferences are considered before the optimization problem is solved (a priori methods) or they are considered during the resolution process. The latter is known as ``interactive'' methods.

\subsubsection{Pareto front navigation}
Preferences are considered when the optimization problem is solved, for example, filtering unfeasible solutions out. It is known as ``a posteriori'' methods.
